Interval Query Problem on Cube-free Median Graphs

In this paper, we introduce the \emph{interval query problem} on cube-free median graphs. Let $G$ be a cube-free median graph and $\mathcal{S}$ be a commutative semigroup. For each vertex $v$ in $G$, we are given an element $p(v)$ in $\mathcal{S}$. For each query, we are given two vertices $u,v$ in $G$ and asked to calculate the sum of $p(z)$ over all vertices $z$ belonging to a $u-v$ shortest path. This is a common generalization of range query problems on trees and grids. In this paper, we provide an algorithm to answer each interval query in $O(\log^2 n)$ time. The required data structure is constructed in $O(n\log^3 n)$ time and $O(n\log^2 n)$ space. To obtain our algorithm, we introduce a new technique, named the \emph{stairs decomposition}, to decompose an interval of cube-free median graphs into simpler substructures.

==> case1-1.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(19.9500,17.4500)(0.0500,-18.0000)%
% LINE 2 0 3 0 Black White  
% 24 2000 1600 2000 1800 2000 1600 1000 1600 1800 1400 1800 1800 1800 1400 1000 1400 1800 1200 1800 1400 1800 1200 1000 1200 1200 1000 1200 1200 1200 1000 1000 1000 1000 1000 1000 1800 1200 1200 1200 1800 1400 1200 1400 1800 1600 1200 1600 1800
% 
\special{pn 8}%
\special{pa 2000 1600}%
\special{pa 2000 1800}%
\special{fp}%
\special{pa 2000 1600}%
\special{pa 1000 1600}%
\special{fp}%
\special{pa 1800 1400}%
\special{pa 1800 1800}%
\special{fp}%
\special{pa 1800 1400}%
\special{pa 1000 1400}%
\special{fp}%
\special{pa 1800 1200}%
\special{pa 1800 1400}%
\special{fp}%
\special{pa 1800 1200}%
\special{pa 1000 1200}%
\special{fp}%
\special{pa 1200 1000}%
\special{pa 1200 1200}%
\special{fp}%
\special{pa 1200 1000}%
\special{pa 1000 1000}%
\special{fp}%
\special{pa 1000 1000}%
\special{pa 1000 1800}%
\special{fp}%
\special{pa 1200 1200}%
\special{pa 1200 1800}%
\special{fp}%
\special{pa 1400 1200}%
\special{pa 1400 1800}%
\special{fp}%
\special{pa 1600 1200}%
\special{pa 1600 1800}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 32 800 600 600 600 800 800 400 800 400 800 400 1200 600 1000 400 1000 800 1000 400 1000 600 1000 400 1000 600 800 600 1200 400 1200 800 1200 600 1200 600 1600 600 1600 800 1600 800 1400 600 1400 600 600 200 600 600 400 600 600 600 400 200 400 200 200 200 600 400 400 400 600
% 
\special{pn 8}%
\special{pa 800 600}%
\special{pa 600 600}%
\special{fp}%
\special{pa 800 800}%
\special{pa 400 800}%
\special{fp}%
\special{pa 400 800}%
\special{pa 400 1200}%
\special{fp}%
\special{pa 600 1000}%
\special{pa 400 1000}%
\special{fp}%
\special{pa 800 1000}%
\special{pa 400 1000}%
\special{fp}%
\special{pa 600 1000}%
\special{pa 400 1000}%
\special{fp}%
\special{pa 600 800}%
\special{pa 600 1200}%
\special{fp}%
\special{pa 400 1200}%
\special{pa 800 1200}%
\special{fp}%
\special{pa 600 1200}%
\special{pa 600 1600}%
\special{fp}%
\special{pa 600 1600}%
\special{pa 800 1600}%
\special{fp}%
\special{pa 800 1400}%
\special{pa 600 1400}%
\special{fp}%
\special{pa 600 600}%
\special{pa 200 600}%
\special{fp}%
\special{pa 600 400}%
\special{pa 600 600}%
\special{fp}%
\special{pa 600 400}%
\special{pa 200 400}%
\special{fp}%
\special{pa 200 200}%
\special{pa 200 600}%
\special{fp}%
\special{pa 400 400}%
\special{pa 400 600}%
\special{fp}%
% LINE 0 2 3 0 Black White  
% 4 1000 1800 800 1800 800 1600 800 1800
% 
\special{pn 20}%
\special{pa 1000 1800}%
\special{pa 800 1800}%
\special{dt 0.045}%
\special{pa 800 1600}%
\special{pa 800 1800}%
\special{dt 0.045}%
% LINE 0 0 3 0 Black White  
% 4 800 800 800 1600 1000 1800 2000 1800
% 
\special{pn 20}%
\special{pa 800 800}%
\special{pa 800 1600}%
\special{fp}%
\special{pa 1000 1800}%
\special{pa 2000 1800}%
\special{fp}%
% LINE 0 2 3 0 Black White  
% 2 800 600 800 800
% 
\special{pn 20}%
\special{pa 800 600}%
\special{pa 800 800}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 12 1000 1000 800 1000 1000 1200 800 1200 1000 1400 800 1400 1000 1600 800 1600 600 600 600 800 400 600 400 800
% 
\special{pn 8}%
\special{pa 1000 1000}%
\special{pa 800 1000}%
\special{dt 0.045}%
\special{pa 1000 1200}%
\special{pa 800 1200}%
\special{dt 0.045}%
\special{pa 1000 1400}%
\special{pa 800 1400}%
\special{dt 0.045}%
\special{pa 1000 1600}%
\special{pa 800 1600}%
\special{dt 0.045}%
\special{pa 600 600}%
\special{pa 600 800}%
\special{dt 0.045}%
\special{pa 400 600}%
\special{pa 400 800}%
\special{dt 0.045}%
% LINE 0 0 3 0 Black White  
% 2 800 1600 800 1800
% 
\special{pn 20}%
\special{pa 800 1600}%
\special{pa 800 1800}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 800 500 800 600 2 0 0 0
% $w$
\put(8.0000,-6.0000){\makebox(0,0)[lb]{$w$}}%
% STR 2 0 3 0 Black White  
% 4 800 1700 800 1800 4 0 0 0
% $t$
\put(8.0000,-18.0000){\makebox(0,0)[rt]{$t$}}%
% STR 2 0 3 0 Black White  
% 4 2000 1700 2000 1800 1 0 0 0
% $v$
\put(20.0000,-18.0000){\makebox(0,0)[lt]{$v$}}%
% STR 2 0 3 0 Black White  
% 4 800 900 800 1000 2 0 0 0
% $e$
\put(8.0000,-10.0000){\makebox(0,0)[lb]{$e$}}%
% STR 2 0 3 0 Black White  
% 4 200 100 200 200 3 0 0 0
% $u$
\put(2.0000,-2.0000){\makebox(0,0)[rb]{$u$}}%
% STR 2 0 3 0 Black White  
% 4 700 1050 700 1100 5 0 0 0
% $L$
\put(7.0000,-11.0000){\makebox(0,0){$L$}}%
% STR 2 0 3 0 Black White  
% 4 1500 1450 1500 1500 5 0 0 0
% $L'$
\put(15.0000,-15.0000){\makebox(0,0){$L'$}}%
\end{picture}}%


==> case1-2.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(25.8000,13.3000)(0.2000,-14.0000)%
% LINE 0 0 3 0 Black White  
% 4 2600 1400 1800 1400 1600 1400 800 1400
% 
\special{pn 20}%
\special{pa 2600 1400}%
\special{pa 1800 1400}%
\special{fp}%
\special{pa 1600 1400}%
\special{pa 800 1400}%
\special{fp}%
% LINE 0 2 3 0 Black White  
% 4 1800 1400 1600 1400 800 1400 600 1400
% 
\special{pn 20}%
\special{pa 1800 1400}%
\special{pa 1600 1400}%
\special{dt 0.045}%
\special{pa 800 1400}%
\special{pa 600 1400}%
\special{dt 0.045}%
% LINE 2 0 3 0 Black White  
% 18 2600 1400 2600 1200 2600 1200 1800 1200 2400 1400 2400 1000 2400 1000 1800 1000 2400 1000 2400 800 2400 800 1800 800 2200 800 2200 1400 2000 800 2000 1400 1800 800 1800 1400
% 
\special{pn 8}%
\special{pa 2600 1400}%
\special{pa 2600 1200}%
\special{fp}%
\special{pa 2600 1200}%
\special{pa 1800 1200}%
\special{fp}%
\special{pa 2400 1400}%
\special{pa 2400 1000}%
\special{fp}%
\special{pa 2400 1000}%
\special{pa 1800 1000}%
\special{fp}%
\special{pa 2400 1000}%
\special{pa 2400 800}%
\special{fp}%
\special{pa 2400 800}%
\special{pa 1800 800}%
\special{fp}%
\special{pa 2200 800}%
\special{pa 2200 1400}%
\special{fp}%
\special{pa 2000 800}%
\special{pa 2000 1400}%
\special{fp}%
\special{pa 1800 800}%
\special{pa 1800 1400}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 52 1600 800 1600 1400 1600 800 1600 600 1600 600 800 600 800 600 800 1400 1200 400 1200 400 1200 600 1200 400 800 400 800 400 800 600 800 400 800 400 1200 400 1000 400 1000 1400 1200 600 1200 1400 1400 800 1400 600 1400 800 1400 1400 1600 800 800 800 1600 1000 800 1000 1600 1200 800 1200 600 1400 600 400 600 1200 400 1200 400 1200 400 400 600 400 200 400 400 400 400 200 400 200 200 200 200 200 200 400 600 600 400 600 600 800 400 800 600 1000 400 1000
% 
\special{pn 8}%
\special{pa 1600 800}%
\special{pa 1600 1400}%
\special{fp}%
\special{pa 1600 800}%
\special{pa 1600 600}%
\special{fp}%
\special{pa 1600 600}%
\special{pa 800 600}%
\special{fp}%
\special{pa 800 600}%
\special{pa 800 1400}%
\special{fp}%
\special{pa 1200 400}%
\special{pa 1200 400}%
\special{fp}%
\special{pa 1200 600}%
\special{pa 1200 400}%
\special{fp}%
\special{pa 800 400}%
\special{pa 800 400}%
\special{fp}%
\special{pa 800 600}%
\special{pa 800 400}%
\special{fp}%
\special{pa 800 400}%
\special{pa 1200 400}%
\special{fp}%
\special{pa 1000 400}%
\special{pa 1000 1400}%
\special{fp}%
\special{pa 1200 600}%
\special{pa 1200 1400}%
\special{fp}%
\special{pa 1400 800}%
\special{pa 1400 600}%
\special{fp}%
\special{pa 1400 800}%
\special{pa 1400 1400}%
\special{fp}%
\special{pa 1600 800}%
\special{pa 800 800}%
\special{fp}%
\special{pa 1600 1000}%
\special{pa 800 1000}%
\special{fp}%
\special{pa 1600 1200}%
\special{pa 800 1200}%
\special{fp}%
\special{pa 600 1400}%
\special{pa 600 400}%
\special{fp}%
\special{pa 600 1200}%
\special{pa 400 1200}%
\special{fp}%
\special{pa 400 1200}%
\special{pa 400 400}%
\special{fp}%
\special{pa 600 400}%
\special{pa 200 400}%
\special{fp}%
\special{pa 400 400}%
\special{pa 400 200}%
\special{fp}%
\special{pa 400 200}%
\special{pa 200 200}%
\special{fp}%
\special{pa 200 200}%
\special{pa 200 400}%
\special{fp}%
\special{pa 600 600}%
\special{pa 400 600}%
\special{fp}%
\special{pa 600 800}%
\special{pa 400 800}%
\special{fp}%
\special{pa 600 1000}%
\special{pa 400 1000}%
\special{fp}%
% LINE 2 2 3 0 Black White  
% 16 1800 800 1600 800 1800 1000 1600 1000 1800 1200 1600 1200 800 1200 600 1200 800 1000 600 1000 800 800 600 800 800 600 600 600 800 400 600 400
% 
\special{pn 8}%
\special{pa 1800 800}%
\special{pa 1600 800}%
\special{dt 0.045}%
\special{pa 1800 1000}%
\special{pa 1600 1000}%
\special{dt 0.045}%
\special{pa 1800 1200}%
\special{pa 1600 1200}%
\special{dt 0.045}%
\special{pa 800 1200}%
\special{pa 600 1200}%
\special{dt 0.045}%
\special{pa 800 1000}%
\special{pa 600 1000}%
\special{dt 0.045}%
\special{pa 800 800}%
\special{pa 600 800}%
\special{dt 0.045}%
\special{pa 800 600}%
\special{pa 600 600}%
\special{dt 0.045}%
\special{pa 800 400}%
\special{pa 600 400}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 2600 1300 2600 1400 1 0 0 0
% $v$
\put(26.0000,-14.0000){\makebox(0,0)[lt]{$v$}}%
% STR 2 0 3 0 Black White  
% 4 600 1300 600 1400 4 0 0 0
% $w$
\put(6.0000,-14.0000){\makebox(0,0)[rt]{$w$}}%
% STR 2 0 3 0 Black White  
% 4 1600 1300 1600 1400 4 0 0 0
% $t$
\put(16.0000,-14.0000){\makebox(0,0)[rt]{$t$}}%
% STR 2 0 3 0 Black White  
% 4 1600 700 1600 800 2 0 0 0
% $e$
\put(16.0000,-8.0000){\makebox(0,0)[lb]{$e$}}%
% STR 2 0 3 0 Black White  
% 4 200 100 200 200 3 0 0 0
% $u$
\put(2.0000,-2.0000){\makebox(0,0)[rb]{$u$}}%
% STR 2 0 3 0 Black White  
% 4 1100 850 1100 900 5 0 0 0
% $L$
\put(11.0000,-9.0000){\makebox(0,0){$L$}}%
% STR 2 0 3 0 Black White  
% 4 2100 1050 2100 1100 5 0 0 0
% $L'$
\put(21.0000,-11.0000){\makebox(0,0){$L'$}}%
\end{picture}}%


==> case2-1.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(17.9500,13.4500)(0.0500,-14.0000)%
% LINE 0 0 3 0 Black White  
% 2 1800 1400 1000 1400
% 
\special{pn 20}%
\special{pa 1800 1400}%
\special{pa 1000 1400}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 16 1600 1400 1600 1200 1600 1200 1000 1200 1600 1200 1600 1000 1600 1000 1000 1000 1400 1400 1400 800 1400 800 1000 800 1200 1400 1200 800 1000 1400 1000 800
% 
\special{pn 8}%
\special{pa 1600 1400}%
\special{pa 1600 1200}%
\special{fp}%
\special{pa 1600 1200}%
\special{pa 1000 1200}%
\special{fp}%
\special{pa 1600 1200}%
\special{pa 1600 1000}%
\special{fp}%
\special{pa 1600 1000}%
\special{pa 1000 1000}%
\special{fp}%
\special{pa 1400 1400}%
\special{pa 1400 800}%
\special{fp}%
\special{pa 1400 800}%
\special{pa 1000 800}%
\special{fp}%
\special{pa 1200 1400}%
\special{pa 1200 800}%
\special{fp}%
\special{pa 1000 1400}%
\special{pa 1000 800}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 6 800 1400 800 1000 800 800 800 400 800 800 400 800
% 
\special{pn 20}%
\special{pa 800 1400}%
\special{pa 800 1000}%
\special{fp}%
\special{pa 800 800}%
\special{pa 800 400}%
\special{fp}%
\special{pa 800 800}%
\special{pa 400 800}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 6 1200 800 1200 600 1000 600 1000 800 1200 600 1000 600
% 
\special{pn 8}%
\special{pa 1200 800}%
\special{pa 1200 600}%
\special{fp}%
\special{pa 1000 600}%
\special{pa 1000 800}%
\special{fp}%
\special{pa 1200 600}%
\special{pa 1000 600}%
\special{fp}%
% LINE 0 2 3 0 Black White  
% 4 1000 1400 800 1400 800 800 800 1000
% 
\special{pn 20}%
\special{pa 1000 1400}%
\special{pa 800 1400}%
\special{dt 0.045}%
\special{pa 800 800}%
\special{pa 800 1000}%
\special{dt 0.045}%
% LINE 2 0 3 0 Black White  
% 26 600 600 800 600 600 600 600 600 600 800 600 600 800 400 400 400 400 400 400 800 600 600 600 400 600 600 400 600 600 400 600 200 600 200 200 200 200 200 200 600 400 600 200 600 400 400 200 400 400 400 400 200
% 
\special{pn 8}%
\special{pa 600 600}%
\special{pa 800 600}%
\special{fp}%
\special{pa 600 600}%
\special{pa 600 600}%
\special{fp}%
\special{pa 600 800}%
\special{pa 600 600}%
\special{fp}%
\special{pa 800 400}%
\special{pa 400 400}%
\special{fp}%
\special{pa 400 400}%
\special{pa 400 800}%
\special{fp}%
\special{pa 600 600}%
\special{pa 600 400}%
\special{fp}%
\special{pa 600 600}%
\special{pa 400 600}%
\special{fp}%
\special{pa 600 400}%
\special{pa 600 200}%
\special{fp}%
\special{pa 600 200}%
\special{pa 200 200}%
\special{fp}%
\special{pa 200 200}%
\special{pa 200 600}%
\special{fp}%
\special{pa 400 600}%
\special{pa 200 600}%
\special{fp}%
\special{pa 400 400}%
\special{pa 200 400}%
\special{fp}%
\special{pa 400 400}%
\special{pa 400 200}%
\special{fp}%
% LINE 2 2 3 0 Black White  
% 8 1000 600 800 600 1000 800 800 800 1000 1000 800 1000 1000 1200 800 1200
% 
\special{pn 8}%
\special{pa 1000 600}%
\special{pa 800 600}%
\special{dt 0.045}%
\special{pa 1000 800}%
\special{pa 800 800}%
\special{dt 0.045}%
\special{pa 1000 1000}%
\special{pa 800 1000}%
\special{dt 0.045}%
\special{pa 1000 1200}%
\special{pa 800 1200}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 1800 1300 1800 1400 1 0 0 0
% $v$
\put(18.0000,-14.0000){\makebox(0,0)[lt]{$v$}}%
% STR 2 0 3 0 Black White  
% 4 800 1300 800 1400 4 0 0 0
% $t$
\put(8.0000,-14.0000){\makebox(0,0)[rt]{$t$}}%
% STR 2 0 3 0 Black White  
% 4 800 700 800 800 4 0 0 0
% $w$
\put(8.0000,-8.0000){\makebox(0,0)[rt]{$w$}}%
% STR 2 0 3 0 Black White  
% 4 800 300 800 400 2 0 0 0
% $w^1$
\put(8.0000,-4.0000){\makebox(0,0)[lb]{$w^1$}}%
% STR 2 0 3 0 Black White  
% 4 200 100 200 200 3 0 0 0
% $u$
\put(2.0000,-2.0000){\makebox(0,0)[rb]{$u$}}%
% STR 2 0 3 0 Black White  
% 4 400 700 400 800 4 0 0 0
% $w^2$
\put(4.0000,-8.0000){\makebox(0,0)[rt]{$w^2$}}%
% STR 2 0 3 0 Black White  
% 4 700 1150 700 1200 5 0 0 0
% $L$
\put(7.0000,-12.0000){\makebox(0,0){$L$}}%
% STR 2 0 3 0 Black White  
% 4 1300 1050 1300 1100 5 0 0 0
% $L'$
\put(13.0000,-11.0000){\makebox(0,0){$L'$}}%
\end{picture}}%

